Hot electron diffusion, microwave noise, and piezoresistivity in Si from first principles

Ab-initio calculations of charge transport properties in materials without adjustable parameters have provided microscopic insights into electron-phonon interactions which govern charge transport properties. Other transport properties such as the diffusion coefficient provide additional microscopic information and are readily accessible experimentally, but few ab-initio calculations of these properties have been performed. Here, we report first-principles calculations of the hot electron diffusion coefficient in Si and its dependence on electric field over temperatures from 77 -- 300 K. While qualitative agreement in trends such as anisotropy at high electric fields is obtained, the quantitative agreement that is routinely achieved for low-field mobility is lacking. We examine whether the discrepancy can be attributed to an inaccurate description of f-type intervalley scattering by computing the microwave-frequency noise spectrum and piezoresistivity. These calculations indicate that any error in the strength of f-type scattering is insufficient to explain the diffusion coefficient discrepancies. Our findings suggest that the measured diffusion coefficient is influenced by factors such as space charge effects which are not included in ab-initio calculations, impacting the interpretation of this property in terms of charge transport processes.

==> scratch.tex <==
% Although the anisotropy with electric field is qualitatively captured at high fields, it is underestimated in magnitude and manifests only at higher fields than are seen in experiment. When calculating the frequency dependence of the PSD and the piezoresistivity, phenomena sensitive to the relative amounts of f-type scattering, we find good agreement with experiment. This suggests that the discrepancy in the PSD versus electric field data is not due to an incorrect description of intervalley scattering, and instead is due to experimental factors not captured in our computation.

%Many theoretical studies of high-field transport and the diffusion coefficient in Si were performed using Monte Carlo methods \cite{Jacoboni_1975,Brunetti_1981,Jacoboni_1983,Pop_2004,Pop_2005,Aksamija_2006,Fischetti_2019}.
%****reduce to super highly cited or review
%These models utilized various approximations, such as dispersionless optical phonons, Debye acoustic phonons, and model bandstructures. Due to the empirical nature of the models, the microscopic causes of noise could not be determined unambiguously. More recently, Monte Carlo work in n-Si has been extended to device simulation \cite{Aksamija_2006} and full-band studies \cite{Fischetti_1991,Fischer_2000, Nguyen_2003,Fischetti_2019}. For most of these studies, different electron-phonon coupling constants were used for the two types of intervalley scattering, g-type (scattering between equivalent valleys) and f-type (scattering between two inequivalent valleys). There existed no definitive conclusion as to the relative strengths of these two, as the available experimental data that was used for comparison were mostly high-field drift velocity curves which are insensitive to the relative amounts of f- and g-type scattering. More recent Monte Carlo methods have investigated the deformation potentials associated with f- and g-type phonons, finding there is a wide range of reported values \cite{Pop_2004}. However, it was shown that intervalley noise is sensitive to the strength of f-type scattering \cite{Brunetti_1981}, which can enable more precise estimates of the strength of each type of scattering. However, no study has been done on n-Si investigating the noise (or the relative amounts of g- and f-type scattering) using ab-initio band structure and scattering rates. 


% . One possible explanation for this is the lack of ionized-impurity scattering in our computation. The addition of ionized-impurity scattering would cause the mobility (and thus, the diffusion coefficient) to decrease, and would become increasingly important at lower temperatures. Another way that including the effect of ionized-impurity scattering would explain some of the discrepancy in experiment in \cref{psd_vs_e_77}, is that with the addition of more scattering channels, the heating of the electron gas will be slowed with electric field, and phenomena seen at lower fields without the inclusion of impurity scattering will be observed at higher fields while including impurity scattering. We posit that the inclusion of impurity scattering would move the peaks seen in our computation in \cref{psd_vs_e_77} to higher fields, giving better agreement with experiment. 



% We note that this underestimation is with including two-phonon scattering, and when only one-phonon scattering is included, the diffusion coefficient we obtain is higher than experiment in this temperature range. This result, where experimental data lies between the computed 1ph and 1+2ph curves is similar to what is observed in the low-field mobility to Si \cite{Hatanpaa_2023}.

% The general underprediction of the magnitude of the anisotropy with respect to experiment would suggest that in our computation, at least for the data between 160 and 300 K, the f-type scattering rates are too large, as the anisotropy is much smaller than experiment. As past studies have shown good agreement when computing transport phenomena that are not sensitive to the specific type (f/g) of scattering, we further investigate other phenomena that are sensitive to this distinction in order to test the validity of this idea.



% The intervalley noise contribution to the PSD that is present with the electric field applied along the [100] direction, but not in the [111], owing to ...

%In order to disaggregate the many types of noise present in a semiconductor away from low fields, investigating the frequency dependence is required, but many experimental and theoretical studies only investigate at a single frequency. The spectral density of current fluctuations has been computed ab-initio previously \cite{Choi_2021}, but here we report the first ab-initio computation with comparison to experimental data.

% This conclusion is at variance with the findings from the results of \Cref{psd_vs_e} in which qualitative discrepancies were observed in the magnitude of intervalley noise between computation and experiment.

%Piezoresistivity has been computed ab-initio for n-Si as a function of biaxial strain \cite{Yu_2008}. Even though it has been shown that in n-Si, applied stress may change the effective mass on the order of 3\% in the stress ranges we are investigating \cite{Yu_2008}, to first order it can be approximated that the largest effects of the applied stress are to change the populations in valleys due to the energy splitting of valleys, and to change the amount of intervalley scattering \cite{Herring_1955}. In order to specifically investigate f-type scattering using piezoresistivity, we can apply compressive stress in the [001] and [011] directions.

%The amounts of f-type scattering for our computations can be checked as well, by looking at the scattering matrix used as an input to the linear solver, and calculating the percentage of the equilibrium-distribution weighted scattering amount that is f-type. At the highest stress calculated, 10.5 kbar, when the stress is applied along the [001] 0.001\% of the scattering is f-type, while when the stress is applied along the [011] 2.43\% of the scattering is f-type (need to re-check these numbers with updated grid). Thus, some of the small difference seen between the two computed curves may be due to this small amount of f-type scattering still present. 

%especially as \cref{psd_vs_e_77} and \cref{psd_vs_f} are at the same temperature of 77 K. However, some of this may be reconciled due to the fact that we do not include ionized-impurity scattering in our computation. The addition of ionized-impurity scattering would cause the momentum relaxation time to decrease, and would become increasingly important at lower temperatures. However, it would not effect the energy relaxation time, as ionized-impurity scattering is elastic and elastic scattering cannot relax energy. In addition, including ionized-impurity scattering would not be expected to appreciably change the intervalley relaxation time, as the transition rate from ionized impurity scattering drops off quickly with increasing angle \cite{Lundstrom_2000}. Thus, it is possible to see good agreement with the spectral data, even when the momentum relaxation time is inaccurately described. There is evidence that this is the case, as at 77 K, the experimental diffusion coefficient is almost an order of magnitude less than the computed value at 77 K. 

%In addition, another explanation for the discrepancy between \cref{psd_vs_e_77} and \cref{psd_vs_f} is that the two data sets used seem to contradict each other. While the diffusion coefficient from \cite{Brunetti_1981} is 160 $\text{cm}^2 \text{s}^{-1}$, the resistivity of the samples used were in the k$\Omega \cdot \text{cm}$ range, while the diffusion coefficients in \cite{Bareikis_1982} were much higher, but with a lower resistivity sample (480 $\Omega \cdot \text{cm}$). We expect the lower resistivity samples (thus less pure) to have a lower mobility, and thus by the Einstein relation, to have a lower diffusion coefficient. This is not the case when comparing the two sets of data, indicating that there is some fundamental disagreement between the two that makes it more difficult to draw conclusions. 

%We find that using our computation, relaxation times are found that are very similar to past experiments \cite{Bareikis_1982,Hartnagel_2001}. Previous Monte Carlo simulation for the [111] configuration gave the energy relaxation time as $\sim$15 ps and the momentum relaxation time as $\sim$2 ps, while our computed results are 10.8 ps and 1.96 ps, respectively. Similarly, the reported energy relaxation and intervalley time were $\sim$5 ps and $\sim$50 ps, while we obtain 4.85 ps and 45.4 ps, respectively.*******these are MC simulations used to interpret the experiments? Like we talked about I hesitate to compare to MC given how many parameters go into them 

Thus, the variation from zero field to the lowest electric field data points is not known, making any choice of normalization somewhat arbitrary.
